Do cavities matter? Hollow microgels resist crystallization

Solutions of microgels have been widely used as model systems to gain insight into atomic condensed matter and complex fluids. We explore the thermodynamic phase behavior of hollow microgels, which are distinguished from conventional colloids by possessing a central cavity. Small-angle neutron and X-ray scattering are used to probe hollow microgels in crowded environments. These measurements reveal an interplay between interpenetration and deswelling, and an unusual absence of crystals. Monte Carlo simulations of hollow microgel solutions confirm that, due to the cavity, they form a supercooled liquid more stable than in the case of microgels with a crosslinked core.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
